Tool-Augmented Reward Modeling

Reward modeling (a.k.a., preference modeling) is instrumental for aligning large language models with human preferences, particularly within the context of reinforcement learning from human feedback (RLHF). While conventional reward models (RMs) have exhibited remarkable scalability, they oft struggle with fundamental functionality such as arithmetic computation, code execution, and factual lookup. In this paper, we propose a tool-augmented preference modeling approach, named Themis, to address these limitations by empowering RMs with access to external environments, including calculators and search engines. This approach not only fosters synergy between tool utilization and reward grading but also enhances interpretive capacity and scoring reliability. Our study delves into the integration of external tools into RMs, enabling them to interact with diverse external sources and construct task-specific tool engagement and reasoning traces in an autoregressive manner. We validate our approach across a wide range of domains, incorporating seven distinct external tools. Our experimental results demonstrate a noteworthy overall improvement of 17.7% across eight tasks in preference ranking. Furthermore, our approach outperforms Gopher 280B by 7.3% on TruthfulQA task in zero-shot evaluation. In human evaluations, RLHF trained with Themis attains an average win rate of 32% when compared to baselines across four distinct tasks. Additionally, we provide a comprehensive collection of tool-related RM datasets, incorporating data from seven distinct tool APIs, totaling 15,000 instances. We have made the code, data, and model checkpoints publicly available to facilitate and inspire further research advancements\footnote{\url{https://github.com/ernie-research/Tool-Augmented-Reward-Model}}.

==> introduction.tex <==

% LLMs waves xxx in various NLP tasks.
% RLHF alignment xxx. Reward model xx important.
% However, limitations:
% 1) outside knowledge
% 2) recency problem
% 3) specific task

% In this paper, ... 
% Contribution:
% 1) construct reward dataset 
% 2) tool-augmented reward model framework, CoTo
% 3) experiment analysis


Large language models (LLMs) trained on vast datasets acquire surprising capabilities~\citep{gpt3,OPT,instrutGPT,GLM,llama},  making substantial strides across various natural language processing tasks, including question answering~\citep{atlas,webgpt}, code generation~\citep{human_eval,codegeex,starcoder}, and general assistance~\citep{instrutGPT,Chameleon}. Nevertheless, foundational LLMs do not consistently yield perfect results and may generate biased content or hallucinated facts that diverge from human expectations~\citep{hallucination_survey}.
Therefore, recent NLP research efforts focus on aligning LLMs with human preferences. One of the most prominent methods is Reinforcement Learning from Human Feedback (RLHF)~\citep{rlhf,summarize_feedback}, a framework that involves learning from human preferences through a reward model trained with human-rated outputs.
Specifically, human labelers are instructed to select one or rank according to their preferences from two or more responses. Subsequently, a reward model is trained with this comparative signal to predict the human-preferred output from the LM-generated sequences. Then the LM is trained with RL to optimize the reward output from the reward model.

The reward model plays a pivotal role in RLHF by providing reward signals that mirror human preferences. However, the conventional reward models exhibit several limitations, as follows:
(1) Human annotators in the RM phrase often integrate external information, employing tools like search engines for knowledge retrieval and validation. In contrast, the trained RMs lack the capability to incorporate external information, which limits their adaptability and knowledge acquisition.
(2) RMs are unable to update their weights after training. This restriction poses a considerable challenge when attempting to access and adapt to more recent information, hindering their ability to stay up-to-date with evolving knowledge.
(3) Conventional RMs encounter difficulties in addressing specific tasks, such as arithmetic reasoning and code execution.
The aforementioned issues highlight the vulnerability of reward models (RMs) in specific domains, where they tend to yield reward scores that are not well-matched to the intended objectives.

To address these challenges, we propose tool-augmented reward modeling, an approach that enhances reward models with the capability to interact with various tools. We first construct a ToolBank, including basic tools for specific tasks, query-based tools to acquire up-to-date information, and knowledge tools to retrieve knowledge. Then we construct a tool-augmented reward dataset (TARA) with ToolBank through multi-agent interactions, and subsequently train a tool-augmented reward model. 

Our main contributions can be summarized as follows:
(1) We release a tool-augmented reward dataset named TARA, including comparison data and tool invocation processes. 
(2) We propose a China-of-Tools (CoTo) method and train a tool-augmented reward model TARM.
(3) We conduct experimental evaluations on our TARA dataset, as well as two downstream datasets, TruthfulQA and Retarded-bar,  convincingly demonstrate the effectiveness of our proposed approach. Furthermore, additional experiments in RLHF underscore the invaluable assistance of our TARM in enhancing the performance of LLMs.
